SA-Occ: Satellite-Assisted 3D Occupancy Prediction in Real World

Existing vision-based 3D occupancy prediction methods are inherently limited in accuracy due to their exclusive reliance on street-view imagery, neglecting the potential benefits of incorporating satellite views. We propose SA-Occ, the first Satellite-Assisted 3D occupancy prediction model, which leverages GPS & IMU to integrate historical yet readily available satellite imagery into real-time applications, effectively mitigating limitations of ego-vehicle perceptions, involving occlusions and degraded performance in distant regions. To address the core challenges of cross-view perception, we propose: 1) Dynamic-Decoupling Fusion, which resolves inconsistencies in dynamic regions caused by the temporal asynchrony between satellite and street views; 2) 3D-Proj Guidance, a module that enhances 3D feature extraction from inherently 2D satellite imagery; and 3) Uniform Sampling Alignment, which aligns the sampling density between street and satellite views. Evaluated on Occ3D-nuScenes, SA-Occ achieves state-of-the-art performance, especially among single-frame methods, with a 39.05% mIoU (a 6.97% improvement), while incurring only 6.93 ms of additional latency per frame. Our code and newly curated dataset are available at https://github.com/chenchen235/SA-Occ.

==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\ifarxiv \crefname{appendix}{App.}{Apps.}
\else \crefname{appendix}{Suppl.}{Suppls.} \fi

\frenchspacing


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/Dynamic-Decoupling.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} ccc|cccc @{}}
\toprule
& DDS & DSA & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1& & & 38.55 & 29.62 & \textbf{54.93}\\
2& \checkmark & & 38.88 (+ 0.33)& 30.27 (+ 0.65) & 54.64\\
3& \checkmark & \checkmark & \textbf{39.05 (+ 0.50)} & \textbf{30.59 (+ 0.97)} & 54.55\\
\bottomrule
\end{tabular}
\caption{Ablation of our Dynamic-Decoupling Fusion. \textbf{DDS}: Dynamic-Decoupling strategy, \textbf{DSA}: spatial attention with dynamic encoding.}
\label{tab:ablation_ddf}
\end{table}

==> tables/ab2.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{2pt}
\fontsize{8.5}{11}\selectfont
\centering
\begin{tabular}{@{} l *{3}{c} @{}}
% Subtable 1
\begin{subtable}[t]{0.55\textwidth}
\centering
\begin{tabular}{@{} cccccccccc @{}}
\toprule
& Model & SAT. & UDS & DDF & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & Baseline \cite{yu2023flashocc} & &  && 32.08 & 23.38 & 48.02\\
2 & - & \checkmark & & & 36.89 (+ 4.81) & 27.40 (+ 4.02) & 54.30 (+ 6.28)\\
3 & - & \checkmark & & \checkmark& 37.16(+ 5.08) & 27.93 (+ 4.45) & 54.07 (+ 6.05)\\
%38.5 & 29.76 & 54.52\\
% 3 & & \checkmark & \checkmark && 38.57 (+ 6.49)& 29.70 (+ 6.32) & \textbf{54.84 (+ 6.82)}\\
4 & - & \checkmark & \checkmark && 38.55 (+ 6.47)& 29.62 (+ 6.24) & \textbf{54.93 (+ 6.91)}\\
% 4 & SA-Occ & \checkmark & \checkmark & \checkmark & \textbf{38.97 (+ 6.89)} & \textbf{30.45 (+ 7.07)}& 54.58 (+ 6.56)\\
5 & SA-Occ (V1) & \checkmark & \checkmark & \checkmark & \textbf{39.05 (+ 6.97)} & \textbf{30.59 (+ 7.21)}& 54.55 (+ 6.53)\\
\bottomrule
\end{tabular}
\caption{\centering Ablation of main structural components. \textbf{SAT.}: overall satellite branch, \textbf{UDS}: Uniformly Distributed Sampling module, \textbf{DDF}: Dynamic-Decoupling Fusion.}
\end{subtable}
\hfill

\begin{subtable}[t]{0.45\textwidth}
    \centering
\begin{tabular}{@{} cc|ccccccccc @{}}
\toprule
& Strategy & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & MaskSegAtt \cite{gao2024complementing} & 23.23 & 8.51 & 50.47\\
2 & Add & 38.57 & 29.70 & 54.84\\
3 & Concat & 38.55 & 29.62 & \textbf{54.93}\\
%38.05\\
% cat align & 37.85 \\
% 4x4 & 37.42 \\
% MaskSegAtt & 37.83\\
% DSF + Align & 38.87 & 30.26 & 54.64\\
% DSF & \textbf{38.97} & \textbf{30.45}& 54.58\\
4 & DDF + Align & 38.78 & 30.13 & 54.63\\
5 & DDF & \textbf{39.05} & \textbf{30.59}& 54.55\\
\bottomrule
\end{tabular}
\caption{\centering Comparative ablation of our Dynamic-Decoupling Fusion and other different fusion methods.}
\end{subtable}

\\ \\
% Subtable 2
\begin{subtable}[t]{0.5\textwidth}
    \centering
\begin{tabular}{@{} cccc|cccccc @{}}
\toprule
& Sat & 2D Sup. & Gate & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & & & & 32.08 & 23.38 & 48.02\\
2 & \checkmark & & &36.6 (+ 4.52) & \textbf{27.48 (+ 4.1)} & 53.22 (+ 5.2)\\
3 & \checkmark & \checkmark& & 36.82 (+ 4.74)& 27.38 (+ 4.0) & 54.13 (+ 6.11)\\
4 & \checkmark & \checkmark& \checkmark& \textbf{36.89 (+ 4.81)} & 27.40 (+ 4.02) & \textbf{54.30 (+ 6.28)}\\
% 1 & & & & 32.08  & 48.02\\
% 2 & \checkmark & & &36.6 (+ 4.52) & 53.22 (+ 5.2)\\
% 3 & \checkmark & \checkmark& & 36.82 (+ 4.74) & 54.13 (+ 6.11)\\
% 4 & \checkmark & \checkmark& \checkmark& \textbf{36.89 (+ 4.81)} & \textbf{54.30 (+ 6.28)}\\
\bottomrule
\end{tabular}
\caption{\centering Ablation of satellite view branch. \textbf{Sat.}: the barely satellite branch, \textbf{2D Sup.}: 2D auxiliary task supervision, \textbf{Gate}: Soft Gate mechanism.}
\end{subtable}
\hfill

\begin{subtable}[t]{0.5\textwidth}
    \centering
\begin{tabular}{@{} ccc|cccc @{}}
\toprule
& DDS & DSA & mIOU (\%) & D mIOU (\%) & S mIOU (\%)
\\
\midrule
1& & & 38.55 & 29.62 & \textbf{54.93}\\
% 2& \checkmark & & 38.91 (+ 0.36)& 30.49 (+ 0.87) & 54.35\\
2& \checkmark & & 38.88 (+ 0.33)& 30.27 (+ 0.65) & 54.64\\
% 3& \checkmark & \checkmark & \textbf{38.97 (+ 0.42)} & \textbf{30.45 (+ 0.83)}& 54.58 (- 0.26)\\
3& \checkmark & \checkmark & \textbf{39.05 (+ 0.50)} & \textbf{30.59 (+ 0.97)} & 54.55\\
\bottomrule
\end{tabular}
\caption{\centering Ablation of our Dynamic-Decoupling Fusion. \textbf{DDS}: Dynamic-Decoupling strategy, \textbf{DSA}: spatial attention with dynamic encoding.}
\end{subtable}

\\ \\
\begin{subtable}[t]{0.5\textwidth}
    \centering
\begin{tabular}{@{} cc|ccc @{}}
\toprule
& Source & mIOU (\%) & D mIOU (\%) & S mIOU (\%)
\\
\midrule
1& 3d occupancy & 37.69 & 30.01 & 51.79\\
2& 3d object box & 37.81 (+ 0.12) & 30.21 (+ 0.2) & 51.74 (- 0.05)\\
3& $1 \cup 2$ & \textbf{37.94 (+ 0.25)} & \textbf{30.29 (+ 0.28)}& \textbf{51.98 (+ 0.19)}\\
\bottomrule
\end{tabular}
\caption{Ablation of dynamic area labels source.}
\end{subtable}

\begin{subtable}[t]{0.5\textwidth}
    \centering
\begin{tabular}{@{} cc|ccc @{}}
\toprule
& Model & FLOPs (G) & Params (M) & Latency (ms) 
\\
\midrule
1& BEVDetOcc (1f) & 241.76 & 29.02 & 149.19\\
2& FlashOcc (M1) & 248.57 & 44.74 & 81.94\\
3& SA-Occ (V1) & 442.19 & 86.43 & 87.58\\
\bottomrule
\end{tabular}
\caption{Ablation of dynamic area labels source.}
\end{subtable}

\end{tabular}
\caption{\centering \label{tab:ab}Ablation study of different components on the nuScenes val set. \textbf{D-mIoU}: Dynamic mIoU, \textbf{S-mIoU}: Static mIoU, \textbf{Bold}: Best.}
\end{table*}


==> tables/dynamic_labels.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} cc|ccc @{}}
\toprule
& Source & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1& 3d occupancy & 37.69 & 30.01 & 51.79\\
2& 3d object box & 37.81 (+ 0.12) & 30.21 (+ 0.2) & 51.74 (- 0.05)\\
3& $1 \cup 2$ & \textbf{37.94 (+ 0.25)} & \textbf{30.29 (+ 0.28)}& \textbf{51.98 (+ 0.19)}\\
\bottomrule
\end{tabular}
\caption{Ablation of dynamic area labels source.}
\label{tab:ablation_labels}
\end{table}

==> tables/fusion.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} cc|ccccccccc @{}}
\toprule
& Strategy & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & MaskSegAtt \cite{gao2024complementing} & 23.23 & 8.51 & 50.47\\
2 & Add & 38.57 & 29.70 & 54.84\\
3 & Concat & 38.55 & 29.62 & \textbf{54.93}\\
4 & DDF + Align & 38.78 & 30.13 & 54.63\\
5 & DDF & \textbf{39.05} & \textbf{30.59}& 54.55\\
\bottomrule
\end{tabular}
\caption{Comparative ablation of our Dynamic-Decoupling Fusion and other different fusion methods.}
\label{tab:ablation_fusion}
\end{table}

==> tables/latency.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} cc|ccc @{}}
\toprule
& Model & FLOPs (G) & Params (M) & Latency (ms) \\
\midrule
1& BEVDetOcc (1f) & 241.76 & 29.02 & 149.19\\
2& FlashOcc (M1) & 248.57 & 44.74 & 81.94\\
3& SA-Occ (V1) & 442.19 & 86.43 & 87.58\\
\bottomrule
\end{tabular}
\caption{Model complexity and latency.}
\label{tab:model_complexity}
\end{table}

==> tables/satellite.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} cccc|cccccc @{}}
\toprule
& Sat & 2D Sup. & Gate & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & & & & 32.08 & 23.38 & 48.02\\
2 & \checkmark & & &36.6 (+ 4.52) & \textbf{27.48 (+ 4.1)} & 53.22 (+ 5.2)\\
3 & \checkmark & \checkmark& & 36.82 (+ 4.74)& 27.38 (+ 4.0) & 54.13 (+ 6.11)\\
4 & \checkmark & \checkmark& \checkmark& \textbf{36.89 (+ 4.81)} & 27.40 (+ 4.02) & \textbf{54.30 (+ 6.28)}\\
\bottomrule
\end{tabular}
\caption{Ablation of satellite view branch. \textbf{Sat.}: the barely satellite branch, \textbf{2D Sup.}: 2D auxiliary task supervision, \textbf{Gate}: Soft Gate mechanism.}
\label{tab:ablation_satellite}
\end{table}

==> tables/structural.tex <==
\begin{table}[!t]
\centering
\fontsize{8.5}{11}\selectfont
\begin{tabular}{@{} ccccccccc @{}}
\toprule
& Model & SAT. & UDS & DDF & mIOU (\%) & D mIOU (\%) & S mIOU (\%)\\
\midrule
1 & Baseline \cite{yu2023flashocc} & &  && 32.08 & 23.38 & 48.02\\
2 & - & \checkmark & & & 36.89 (+ 4.81) & 27.40 (+ 4.02) & 54.30 (+ 6.28)\\
3 & - & \checkmark & & \checkmark& 37.16(+ 5.08) & 27.93 (+ 4.45) & 54.07 (+ 6.05)\\
4 & - & \checkmark & \checkmark && 38.55 (+ 6.47)& 29.62 (+ 6.24) & \textbf{54.93 (+ 6.91)}\\
5 & SA-Occ (V1) & \checkmark & \checkmark & \checkmark & \textbf{39.05 (+ 6.97)} & \textbf{30.59 (+ 7.21)}& 54.55 (+ 6.53)\\
\bottomrule
\end{tabular}
\caption{Ablation of main structural components. \textbf{SAT.}: overall satellite branch, \textbf{UDS}: Uniformly Distributed Sampling module, \textbf{DDF}: Dynamic-Decoupling Fusion.}
\label{tab:ablation_structural}
\end{table}
